ArCo: the Italian Cultural Heritage Knowledge Graph

ArCo is the Italian Cultural Heritage knowledge graph, consisting of a network of seven vocabularies and 169 million triples about 820 thousand cultural entities. It is distributed jointly with a SPARQL endpoint, a software for converting catalogue records to RDF, and a rich suite of documentation material (testing, evaluation, how-to, examples, etc.). ArCo is based on the official General Catalogue of the Italian Ministry of Cultural Heritage and Activities (MiBAC) - and its associated encoding regulations - which collects and validates the catalogue records of (ideally) all Italian Cultural Heritage properties (excluding libraries and archives), contributed by CH administrators from all over Italy. We present its structure, design methods and tools, its growing community, and delineate its importance, quality, and impact.

==> sections/issues.tex <==
Figure \ref{img:record} %\todo{aggiungere caption}
depicts a painting by \href{https://en.wikipedia.org/wiki/Albert_J._Friscia}{Albert Friscia} with some excerpts from its XML catalogue record. 
%In each XML snippet we provide an English translation of values. 
%The complete \href{http://www.catalogo.beniculturali.it/sigecSSU_FE/schedaCompleta.action?keycode=ICCD11313702}{catalogue record} includes 63 descriptive files, some of which have nested attributes. 
%
\begin{figure}[ht!] \centering
%\includegraphics[width=1.3\textwidth,angle=90]{img/painting-draft.png}
\includegraphics[width=\textwidth,scale=0.40]{img/painting-draft.png}
	\caption{An example of XML data from ICCD Catalogue. Each snippet is translated to English.}
	\label{img:record}
\end{figure}
%
The first issue with XML data is that all information in the records is expressed as strings. In order to build a RDF KG, good practice suggests to produce individuals for every element (or set of elements), whose value (or set of values) refers to anything that may participate as a subject in a triple, or can be linked to, or from, external resources. For example, we want to create an individual for Albert Friscia (the author), as well as an individual for the technical status of this painting. As part of the modeling process (cf. Section \ref{sec:ontology}), we define ArCo classes by abstracting from sets of fields and we define rules for creating URIs for their individuals %which are used in the XML to RDF conversion 
(cf. Section \ref{sec:method}).
%the classes defined within the ArCo ontology network. Those classes can be briefly listed by using the those defined in the \href{https://w3id.org/italia/onto/l0/}{Level-0} (L0) ontology. L0 is the top-level designed for modelling the ontology network of the Italian Public Administration. Hence, L0 is also the top-level of the ArCo ontology network. In fact, all the classes and properties defined into the ArCo modules are aligned to L0 classes and properties by means of \texttt{rdfs:subClassOf} and \texttt{rdfs:subPropertyOf} aximos, respectively. Namely, the classes of L0 that we instantiate are:
%\texttt{Activity}, \texttt{Agent}, \texttt{Characteristic}, \texttt{Collection}, \texttt{Concept}, \texttt{Description}, \texttt{Entity}, \texttt{EventOrSituation}, \texttt{Location}, \texttt{Object}, and \texttt{Topic}.
\noindent{\bf URI production.} ArCo base URI for individuals is \texttt{https://w3id.org/arco/resource/} with prefix  \texttt{data:}. Every individual's ID is preceded by the name of its type. An individual's ID can be produced in three ways. If the individual can be disambiguated by the value of one element, we use that value. Otherwise, we either concatenate the values of more elements, or when unfeasible we compute a MD5 checksum from the values of some selected elements %(when concatenating is unfeasible). 
For example, referring to Figure \ref{img:record}, the URI of the author Albert Friscia is \texttt{data:Agent/albert-friscia-attivo-dal-1935-al-1989}, obtained by concatenating his name (element \texttt{AUTN}) and his biographical data (element \texttt{AUTA}). As another example, for the ID of the technical status of a painting of his, we generate the URI \texttt{data:CPTechnicalStatus/1700168650}, where 1700168650 is the painting unique identifier obtained by concatenating the content of \texttt{NCTR} (region code) and \texttt{NCTN} (general catalogue identifier).
\todo[inline]{@Andrea: controlliamo perché le URI non risolvono\\ @Aldo: occhio questo metodo sembra codificare l'opera, non il suo status tecnico!}
%can be the result of the concatenation of more than one value
%to produce URIs having the type an entity belongs to as part of the URI of such an entity. This is done by concatenating the base URI of ArCo resources (i.e. \texttt{https://w3id.org/arco/resource/}) with the local name of the class used for typing the specific entity we want to generate a URI for. For example, an entity whose type is \texttt{arco:ArchaeologicalProperty} produces the namespace \texttt{https://w3id.org/arco/resource/ArchaeologicalProperty/}. 
%Then for generating the local name of the URIs from the text content of the XML elements we distinguish three different cases. Namely, (i) a URI is produced from a single XML element. For example, the element \texttt{<PVCC>Roma</PVCC>} produces the URI \texttt{https://w3id.org/arco/resource/City/roma}; (ii) a URI is produced by concatenating the content of multiple selected elements. For example, the values \texttt{<NCTR>12</NCTR>} and 
%\texttt{<NCTN>00580016</NCTN>} produce the URI \texttt{https://w3id.org/arco/resource/CatalogueRecordRA/1200580016}; and (iii) a URI is obtained by computing the MD5 checksum from the content of selected elements. For example, the elements \texttt{<PRVR>Piemonte</PRVR>}, \texttt{<PRVP>VC</PRVP>}, \texttt{<PRVC>Trino</PRVC>}, \texttt{<PRCT>chiesa</PRCT>}, \texttt{<PRCQ>parrocchiale</PRCQ>}, and \texttt{<PRCS>Oratorio</PRCS>} identifies the site a cultural property is located in. Hence, the resulting URI is \texttt{https://w3id.org/arco/resource/Site/17a15797226b13c28694435a4927e440}. The MD5 allows to have concise URIs from long and complex text content. The direct use of string content for generating URIs might introduce homonyms or duplicates, but a data cleaning step ease the issue. It is worth saying that we do not have a data cleaning step for homonym or duplicate entities. Nevertheless, we aim at reusing solution like~\cite{Zhang2017} in our future work.

\noindent{\bf Modeling issues.} Typical modeling issues encountered during the design of ArCo firstly concern requirements about explicit representation of many type-specific, detailed characteristics of cultural properties. While existing CH ontologies allow specialisation of their types, e.g. EDM \texttt{Aggregation} collects all metadata of a cultural entity, in our case a stronger ontological commitment is taken to deal with alignment to existing ontologies in order to facilitate reuse and enrichment. For example, a museum may use EDM \texttt{Aggregation}, but may exploit at the same time the richness of ArCo ontologies for specialising it. The general modeling choices adopted in ArCo are described in Section \ref{sec:ontology}. 

Another requirement that impacted our modeling approach is to express a same concept both with highly expressive \emph{n-ary} relation patterns, and \emph{shortcut} binary relations, which support light weight modeling. For example, for representing the material of a cultural property ArCo has both a binary relation \texttt{:hasMaterial} and a class \texttt{:CulturalEntityTechnicalStatus}, a \emph{n-ary} relation including material among its arguments. ArCo offers both models for most of its types. The link between detailed and lightweight models is provided by property chain axioms, as explained later (for details, cf. \cite{Lodi2017}).  
